FALCON: Honest-Majority Maliciously Secure Framework for Private Deep Learning

We propose Falcon, an end-to-end 3-party protocol for efficient private training and inference of large machine learning models. Falcon presents four main advantages - (i) It is highly expressive with support for high capacity networks such as VGG16 (ii) it supports batch normalization which is important for training complex networks such as AlexNet (iii) Falcon guarantees security with abort against malicious adversaries, assuming an honest majority (iv) Lastly, Falcon presents new theoretical insights for protocol design that make it highly efficient and allow it to outperform existing secure deep learning solutions. Compared to prior art for private inference, we are about 8x faster than SecureNN (PETS'19) on average and comparable to ABY3 (CCS'18). We are about 16-200x more communication efficient than either of these. For private training, we are about 6x faster than SecureNN, 4.4x faster than ABY3 and about 2-60x more communication efficient. Our experiments in the WAN setting show that over large networks and datasets, compute operations dominate the overall latency of MPC, as opposed to the communication.

==> Figures/AlexNet.tex <==

\begin{figure}[H]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|c|}
%\hline
Layer	& Input Size & Description & Output	\\ \hline\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $11 \times 11$, Stride $(4, 4)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$32 \times 32 \times 3$}  &  Padding $(9,9)$, output channels $96$ & \multirow{-2}{*}{$11 \times 11 \times 96$}\\ \hline

%\rowcolor{gray!20} Convolution	& $32 \times 32 \times 3$  &  Window size $11 \times 11$, Stride $(4, 4)$, Padding $(9, 9)$, output channels $96$ & $11 \times 11 \times 96$	\\ \hline

ReLU Activation	&  $11 \times 11 \times 96$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $11 \times 11 \times 96$	\\ \hline

Max Pooling	& $11 \times 11 \times 96$	& Window size $3 \times 3$, Stride $(2,2)$ & $5 \times 5 \times 96$	\\ \hline

 & &  Normalization and linear scaling & \\

 \multirow{-2}{*}{Batch Normalization}	& \multirow{-2}{*}{$5 \times 5 \times 96$}  &  using learnable parameters $\gamma, \beta$  & \multirow{-2}{*}{ $5 \times 5 \times 96$}\\ \hline

%Batch Normalization & $5 \times 5 \times 96$ & Normalization and linear scaling using learnable parameters $\gamma, \beta$ & $5 \times 5 \times 96$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $5 \times 5$, Stride $(1,1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$5 \times 5 \times 96$}  &  Padding $(1,1)$, output channels $256$ & \multirow{-2}{*}{$3 \times 3 \times 256$}\\ \hline

%\rowcolor{gray!20} Convolution	& $5 \times 5 \times 96$  &  Window size $5 \times 5$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $256$ & $3 \times 3 \times 256$	\\ \hline

ReLU Activation	&  $3 \times 3 \times 256$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $3 \times 3 \times 256$	\\ \hline

Max Pooling	& $3 \times 3 \times 256$	& Window size $3 \times 3$, Stride $(2,2)$ & $1 \times 1 \times 256$	\\ \hline


 & &  Normalization and linear scaling & \\

 \multirow{-2}{*}{Batch Normalization}	& \multirow{-2}{*}{$1 \times 1 \times 256$}  &  using learnable parameters $\gamma, \beta$  & \multirow{-2}{*}{ $1 \times 1 \times 256$}\\ \hline

%Batch Normalization & $1 \times 1 \times 256$ & Normalization and linear scaling using learnable parameters $\gamma, \beta$ & $1 \times 1 \times 256$	\\ \hline


%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1,1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$1 \times 1 \times 256$}  &  Padding $(1,1)$, output channels $384$ & \multirow{-2}{*}{$1 \times 1 \times 384$}\\ \hline

%\rowcolor{gray!20} Convolution	& $1 \times 1 \times 256$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $384$ & $1 \times 1 \times 384$	\\ \hline

ReLU Activation	&  $1 \times 1 \times 384$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $1 \times 1 \times 384$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1,1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$1 \times 1 \times 384$}  &  Padding $(1,1)$, output channels $384$ & \multirow{-2}{*}{$1 \times 1 \times 384$}\\ \hline

%\rowcolor{gray!20} Convolution	& $1 \times 1 \times 384$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $384$ & $1 \times 1 \times 384$	\\ \hline

ReLU Activation	&  $1 \times 1 \times 384$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $1 \times 1 \times 384$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1,1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$1 \times 1 \times 384$}  &  Padding $(1,1)$, output channels $256$ & \multirow{-2}{*}{$1 \times 1 \times 256$}\\ \hline

%\rowcolor{gray!20} Convolution	& $1 \times 1 \times 384$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $256$ & $1 \times 1 \times 256$	\\ \hline

ReLU Activation	&  $1 \times 1 \times 256$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $1 \times 1 \times 256$	\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} Fully Connected Layer & $256$ & Fully connected layer & $256$	\\ \hline

ReLU Activation	& $256$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $256$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $256$ & Fully connected layer & $256$	\\ \hline

ReLU Activation	& $256$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $256$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $256$ & Fully connected layer & $10$	\\ \hline

ReLU Activation	& $10$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $10$	\\ %\hline
\end{tabular}
}
\caption{AlexNet network architecture~\cite{alexnet} for training over CIFAR-10 dataset.}\label{fig:alexnet}
\end{figure}



==> Figures/LeNet.tex <==

\begin{figure}[H]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|c|}
%\hline
Layer	& Input Size & Description & Output	\\ \hline\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $5 \times 5$, Stride $(1, 1)$, & \\ 

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$28 \times 28 \times 1$}  &  Padding $(0, 0)$, output channels $20$ & \multirow{-2}{*}{$24 \times 24 \times 20$}\\ \hline

%\rowcolor{gray!20} Convolution	& $28 \times 28 \times 1$  &  Window size $5 \times 5$, Stride $(1, 1)$, Padding $(0, 0)$, output channels $20$ & $24 \times 24 \times 20$	\\ \hline

ReLU Activation	&  $24 \times 24 \times 20$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $24 \times 24 \times 20$	\\ \hline

Max Pooling	& $24 \times 24 \times 20$	& Window size $2 \times 2$, Stride $(2,2)$ & $12 \times 12 \times 20$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $5 \times 5$, Stride $(1, 1)$,  & \\ 

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$12 \times 12 \times 20$}  &  Padding $(0, 0)$, output channels $50$ & \multirow{-2}{*}{$8 \times 8 \times 50$}\\ \hline

%\rowcolor{gray!20} Convolution	& $12 \times 12 \times 20$  &  Window size $5 \times 5$, Stride $(1, 1)$, Padding $(0, 0)$, output channels $50$ & $8 \times 8 \times 50$	\\ \hline

ReLU Activation	&  $8 \times 8 \times 50$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $8 \times 8 \times 50$	\\ \hline

Max Pooling	& $8 \times 8 \times 50$	& Window size $2 \times 2$, Stride $(2,2)$ & $4 \times 4 \times 50$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} Fully Connected Layer & $800$ & Fully connected layer & $500$	\\ \hline

ReLU Activation	& $500$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $500$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $500$ & Fully connected layer & $10$	\\ \hline

ReLU Activation	& $10$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $10$	\\ %\hline
\end{tabular}
}
\caption{LeNet network architecture~\cite{lenet} for training over MNIST dataset.}\label{fig:lenet}
\end{figure}



==> Figures/MiniONN.tex <==

\begin{figure}[H]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|c|}
%\hline
Layer	& Input Size & Description & Output	\\ \hline\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $5 \times 5$, Stride $(1, 1)$, & \\ 

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$28 \times 28 \times 1$}  &  Padding $(0, 0)$, output channels $16$ & \multirow{-2}{*}{$24 \times 24 \times 16$}\\ \hline

%\rowcolor{gray!20} Convolution	& $28 \times 28 \times 1$  &  Window size $5 \times 5$, Stride $(1, 1)$, Padding $(0, 0)$, output channels $16$ & $24 \times 24 \times 16$	\\ \hline

ReLU Activation	&  $24 \times 24 \times 16$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $24 \times 24 \times 16$	\\ \hline

Max Pooling	& $24 \times 24 \times 16$	& Window size $2 \times 2$, Stride $(2,2)$ & $12 \times 12 \times 16$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $5 \times 5$, Stride $(1, 1)$,  & \\ 

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$12 \times 12 \times 16$}  &  Padding $(0, 0)$, output channels $16$ & \multirow{-2}{*}{$8 \times 8 \times 16$}\\ \hline

%\rowcolor{gray!20} Convolution	& $12 \times 12 \times 16$  &  Window size $5 \times 5$, Stride $(1, 1)$, Padding $(0, 0)$, output channels $16$ & $8 \times 8 \times 16$	\\ \hline

ReLU Activation	&  $8 \times 8 \times 16$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $8 \times 8 \times 16$	\\ \hline

Max Pooling	& $8 \times 8 \times 16$	& Window size $2 \times 2$, Stride $(2,2)$ & $4 \times 4 \times 16$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} Fully Connected Layer & $256$ & Fully connected layer & $100$	\\ \hline

ReLU Activation	& $100$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $100$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $100$ & Fully connected layer & $10$	\\ \hline

ReLU Activation	& $10$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $10$	\\ %\hline
\end{tabular}
}
\caption{Neural network architecture used in MiniONN~\cite{minionn} for training over MNIST dataset.}\label{fig:minionn}
\end{figure}



==> Figures/Sarda.tex <==

\begin{figure}[H]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|c|}
%\hline
Layer	& Input Size & Description & Output	\\ \hline\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\rowcolor{gray!20} Convolution	& $28 \times 28 \times 1$  &  Window size $2 \times 2$, Stride $(2, 2)$, Padding $(0, 0)$, output channels $5$ & $14 \times 14 \times 5$	\\ \hline

\rowcolor{gray!20} & &  Window size $2 \times 2$, Stride $(2, 2)$, & \\ 

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$28 \times 28 \times 1$}  &  Padding $(0, 0)$, output channels $5$ & \multirow{-2}{*}{$14 \times 14 \times 5$}\\ \hline

ReLU Activation	&  $14 \times 14 \times 5$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $14 \times 14 \times 5$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} Fully Connected Layer & $980$ & Fully connected layer & $100$	\\ \hline

ReLU Activation	& $100$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $100$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $100$ & Fully connected layer & $10$	\\ \hline

ReLU Activation	& $10$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $10$	\\ %\hline
\end{tabular}
}
\caption{Neural network architecture used in Chameleon~\cite{chameleon} for training over MNIST dataset.}\label{fig:chameleon}
\end{figure}



==> Figures/SecureML.tex <==

\begin{figure}[H]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|c|}
%\hline
Layer	& Input Size & Description & Output	\\ \hline\hline


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} Fully Connected Layer & $28 \times 28$ & Fully connected layer & $128$	\\ \hline

ReLU Activation	& $128$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $128$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $128$ & Fully connected layer & $128$	\\ \hline

ReLU Activation	& $128$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $128$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $128$ & Fully connected layer & $10$	\\ \hline

ReLU Activation	& $10$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $10$	\\ %\hline
\end{tabular}
}
\caption{Neural Network architecture from SecureML~\cite{secureml} for training over MNIST dataset.}\label{fig:secureml}
\end{figure}



==> Figures/VGG16.tex <==

\begin{figure}[H]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|c|}
%\hline
Layer	& Input Size & Description & Output	\\ \hline\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$32 \times 32 \times 3$}  &  Padding $(1, 1)$, output channels $64$ & \multirow{-2}{*}{$32 \times 32 \times 64$}\\ \hline

%\rowcolor{gray!20} Convolution	& $32 \times 32 \times 3$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $64$ & $32 \times 32 \times 64$	\\ \hline

ReLU Activation	&  $32 \times 32 \times 64$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $32 \times 32 \times 64$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$32 \times 32 \times 64$}  &  Padding $(1,1)$, output channels $64$ & \multirow{-2}{*}{$32 \times 32 \times 64$}\\ \hline

%\rowcolor{gray!20} Convolution	& $32 \times 32 \times 64$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $64$ & $32 \times 32 \times 64$	\\ \hline

ReLU Activation	&  $32 \times 32 \times 64$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $32 \times 32 \times 64$	\\ \hline

Max Pooling	& $32 \times 32 \times 64$	& Window size $2 \times 2$, Stride $(2,2)$ & $16 \times 16 \times 64$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$16 \times 16 \times 64$}  &  Padding $(1,1)$, output channels $128$ & \multirow{-2}{*}{$16 \times 16 \times 128$	}\\ \hline

%\rowcolor{gray!20} Convolution	& $16 \times 16 \times 64$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $128$ & $16 \times 16 \times 128$	\\ \hline

ReLU Activation	&  $16 \times 16 \times 128$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $16 \times 16 \times 128$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$16 \times 16 \times 128$	}  &  Padding $(1,1)$, output channels $128$ & \multirow{-2}{*}{$16 \times 16 \times 128$	}\\ \hline

%\rowcolor{gray!20} Convolution	& $16 \times 16 \times 128$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $128$ & $16 \times 16 \times 128$	\\ \hline

ReLU Activation	& $16 \times 16 \times 128$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $16 \times 16 \times 128$	\\ \hline

Max Pooling	& $16 \times 16 \times 128$	& Window size $2 \times 2$, Stride $(2,2)$ & $8 \times 8 \times 128$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$8 \times 8 \times 128$	}  &  Padding $(1,1)$, output channels $256$ & \multirow{-2}{*}{$8 \times 8 \times 256$}\\ \hline

%\rowcolor{gray!20} Convolution	& $8 \times 8 \times 128$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $256$ & $8 \times 8 \times 256$	\\ \hline

ReLU Activation	&  $8 \times 8 \times 256$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $8 \times 8 \times 256$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$8 \times 8 \times 256$}  &  Padding $(1,1)$, output channels $256$ & \multirow{-2}{*}{$8 \times 8 \times 256$}\\ \hline

%\rowcolor{gray!20} Convolution	& $8 \times 8 \times 256$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $256$ & $8 \times 8 \times 256$	\\ \hline

ReLU Activation	& $8 \times 8 \times 256$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $8 \times 8 \times 256$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$8 \times 8 \times 256$}  &  Padding $(1,1)$, output channels $256$ & \multirow{-2}{*}{$8 \times 8 \times 256$}\\ \hline

%\rowcolor{gray!20} Convolution	& $8 \times 8 \times 256$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $256$ & $8 \times 8 \times 256$	\\ \hline

ReLU Activation	& $8 \times 8 \times 256$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $8 \times 8 \times 256$	\\ \hline

Max Pooling	& $8 \times 8 \times 256$	& Window size $2 \times 2$, Stride $(2,2)$ & $4 \times 4 \times 256$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$4 \times 4 \times 256$}  &  Padding $(1,1)$, output channels $512$ & \multirow{-2}{*}{$4 \times 4 \times 512$}\\ \hline

%\rowcolor{gray!20} Convolution	& $4 \times 4 \times 256$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $512$ & $4 \times 4 \times 512$	\\ \hline

ReLU Activation	&  $4 \times 4 \times 512$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $4 \times 4 \times 512$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$4 \times 4 \times 512$}  &  Padding $(1,1)$, output channels $512$ & \multirow{-2}{*}{$4 \times 4 \times 512$}\\ \hline

%\rowcolor{gray!20} Convolution	& $4 \times 4 \times 512$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $512$ & $4 \times 4 \times 512$	\\ \hline

ReLU Activation	& $4 \times 4 \times 512$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $4 \times 4 \times 512$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$4 \times 4 \times 512$}  &  Padding $(1,1)$, output channels $512$ & \multirow{-2}{*}{$4 \times 4 \times 512$}\\ \hline

%\rowcolor{gray!20} Convolution	& $4 \times 4 \times 512$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $512$ & $4 \times 4 \times 512$	\\ \hline

ReLU Activation	& $4 \times 4 \times 512$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $4 \times 4 \times 512$	\\ \hline

Max Pooling	& $4 \times 4 \times 512$	& Window size $2 \times 2$, Stride $(2,2)$ & $2 \times 2 \times 512$	\\ \hline

%\multicolumn{4}{c}{~} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$2 \times 2 \times 512$}  &  Padding $(1, 1)$, output channels $512$ & \multirow{-2}{*}{$2 \times 2 \times 512$}\\ \hline

%\rowcolor{gray!20} Convolution	& $2 \times 2 \times 512$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $512$ & $2 \times 2 \times 512$	\\ \hline

ReLU Activation	&  $2 \times 2 \times 512$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $2 \times 2 \times 512$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\ 

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$2 \times 2 \times 512$}  &  Padding $(1, 1)$, output channels $512$ & \multirow{-2}{*}{$2 \times 2 \times 512$}\\ \hline

%\rowcolor{gray!20} Convolution	&$2 \times 2 \times 512$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $512$ & $2 \times 2 \times 512$	\\ \hline

ReLU Activation	& $2 \times 2 \times 512$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $2 \times 2 \times 512$	\\ \hline

\rowcolor{gray!20} & &  Window size $3 \times 3$, Stride $(1, 1)$, & \\ 

\rowcolor{gray!20} \multirow{-2}{*}{Convolution}	& \multirow{-2}{*}{$2 \times 2 \times 512$}  &  Padding $(1, 1)$, output channels $512$ & \multirow{-2}{*}{$2 \times 2 \times 512$}\\ \hline

%\rowcolor{gray!20} Convolution	& $2 \times 2 \times 512$  &  Window size $3 \times 3$, Stride $(1, 1)$, Padding $(1, 1)$, output channels $512$ & $2 \times 2 \times 512$	\\ \hline

ReLU Activation	& $2 \times 2 \times 512$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $2 \times 2 \times 512$	\\ \hline

Max Pooling	& $2 \times 2 \times 512$	& Window size $2 \times 2$, Stride $(2,2)$ & $1 \times 1 \times 512$	\\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{gray!20} Fully Connected Layer & $512$ & Fully connected layer & $4096$	\\ \hline

ReLU Activation	& $4096$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $4096$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $4096$ & Fully connected layer & $4096$	\\ \hline

ReLU Activation	& $4096$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $4096$	\\ \hline

\rowcolor{gray!20} Fully Connected Layer & $4096$ & Fully connected layer & $1000$	\\ \hline

ReLU Activation	& $1000$	 &  $\mathsf{ReLU}(\cdot)$ on each input &  $1000$	\\ %\hline
\end{tabular}
}
\caption{VGG16 network architecture~\cite{vgg16} for training over CIFAR-10 dataset.}\label{fig:VGG16}
\end{figure}



==> Functionalities/func-prep.tex <==

\begin{Boxfig}{Ideal functionality for \protx{Prep}}{FPrep}{$\Funct{Prep}$}

\protx{Prep} generates all the required correlated randomness required by the various functionalities. $\Funct{Prep}$ \\

$\mathsf{GenMAC}(a, \Delta, \alpha)$: This subroutine will be called multiple times by the functionality.
    \begin{enumerate}[nolistsep]
        \item Receive MAC shares $\{\gamma^i\}_{i \in \mathcal{A}}$ from the adversary
        \item Set $\gamma(a) \leftarrow \alpha \cdot a$ and $\gamma \leftarrow \gamma(a) + \Delta$
        \item Sample random values for $\gamma(a)^i \xleftarrow{r} \mathbb{Z}_p$ for $i \notin \mathcal{A}$ subject to $\gamma = \sum_{i=1}^n \gamma(a)^i$
        \item Return $\gamma(a)^i$ to party $P_i$ for $i \notin \mathcal{A}$
    \end{enumerate}
    
\begin{description}
\item[Initialize:]On input $(\mathsf{init,} p)$ from all the parties, do the following: 
    \begin{enumerate}
        \item Receive share $\alpha^i$ from the adversary for $i \in \mathcal{A}$ and sample $\alpha^i \xleftarrow{r} \mathbb{Z}_p$ for each $i \notin \mathcal{A}$. Set $\alpha \leftarrow \alpha^1 + \hdots \alpha^n \pmod{p}$
        \item Wait for $\mathsf{Ok}$ or $\mathsf{Abort}$ from the adversary. If the adversary sends $\mathsf{Abort}$, send $\mathsf{Abort}$ to all parties and abort otherwise send $\alpha^i$ to party $P_i$.
    \end{enumerate}

\item[Authenticated Singles: ]On receiving input $(\mathsf{Authenticated~Singles})$ from all parties, do the following:
    \begin{enumerate}
        \item Wait for $\mathsf{Ok}$ or $\mathsf{Abort}$ from the adversary. If the adversary sends $\mathsf{Abort}$, send $\mathsf{Abort}$ to all parties and abort. Otherwise choose random values $r^i_k \in \mathbb{Z}_p$ for $i \notin \mathcal{A}$ and send them to $P_i$ for all $i \notin \mathcal{A}$
        \item For each corrupt party $P_i, i \in \mathcal{A}$, the adversary specifies a share $r^i$
        \item The environment specifies MAC errors $\Delta_k$. Let $r_k = \sum_i r^i_k$
        \item Run the Macro $\mathsf{GenMAC}(r_k, \Delta_k, \alpha)$
    \end{enumerate}
    
\item[Matrix Triples: ]On receiving input $(\mathsf{Matrix~Triples}, d_1, d_2, d_3)$ from all parties, do the following:
    \begin{enumerate}
        \item Wait for $\mathsf{Ok}$ or $\mathsf{Abort}$ from the adversary. If the adversary sends $\mathsf{Abort}$, send $\mathsf{Abort}$ to all parties and abort. Otherwise choose random matrices $A^i \leftarrow U(R_p)^{d_1\times d_2}$ and $B^i \leftarrow U(R_p)^{d_2\times d_3}$.
        \item For each corrupt party $P_i, i \in A$, the environment specifies shares $A^i \leftarrow U(R_p)^{d_1\times d_2}$, $B^i \leftarrow U(R_p)^{d_2\times d_3}$, and $C^i \leftarrow U(R_p)^{d_1\times d_3}$
        \item The environment specifies the  MAC errors $\Delta_A, \Delta_B$ and $\Delta_C$
        \item Set $A = \sum_i A^i, B = \sum_i B^i$ and $C = A \times B + \delta_{AB}$ 
        \item For each honest party $P_i, i\notin \mathcal{A}$ randomly choose $C^i$ subject to $C = \sum_i C^i$ 
        \item Run Macros $\mathsf{GenMAC}(A, \Delta_A, \alpha), \mathsf{GenMAC}( B, \Delta_B, \alpha)$ and $\mathsf{GenMAC}((A \times B), \Delta_C, \alpha)$
    \end{enumerate}

\item[Convolution Triples: ]Let $\circledast$ denote the 2D-convolution operation. On receiving input $\mathsf{Convolution~Triples}$ along with the convolutions, do the following:
   \begin{enumerate}
        \item Wait for $\mathsf{Ok}$ or $\mathsf{Abort}$ from the adversary. If the adversary sends $\mathsf{Abort}$, send $\mathsf{Abort}$ to all parties and abort. Otherwise choose random matrices $X^i, Y^i$ of given dimensions.
        \item Environment specifies shares $X^i, Y^i, Z^i$ for $i\in \mathcal{A}$. 
        \item Compute $Z = X \circledast Y$, where $X \leftarrow \sum_i X^i$ and $Y \leftarrow \sum_i Y^i$
        \item Generate shares for honest parties such that $Z = \sum_i Z^i$
        \item Run Macros $\mathsf{GenMAC}(X, 0, \alpha), \mathsf{GenMAC}(Y, 0, \alpha)$ and $\mathsf{GenMAC}(Z, 0, \alpha)$
        % \item For each corrupt party $P_i, i \in \mathcal{A}$, the environment specifies shares $X^i, Y^i$, and $Z^i$
        % \item The environment specifies the  MAC errors $\Delta_X, \Delta_Y$ and $\Delta_Z$
        % \item Set $X = \sum_i X^i, Y = \sum_i Y^i$ and $Z = X \circledast Y + \delta_{XY}$ 
        % \item For each honest party $P_i, i\notin \mathcal{A}$ randomly choose $C^i$ subject to $C = \sum_i C^i$ 
        % \item Run Macros $\mathsf{GenMAC}(X, \Delta_X, \alpha), \mathsf{GenMAC}( Y, \Delta_Y, \alpha)$ and $\mathsf{GenMAC}((X \circledast Y), \Delta_C, \alpha)$
    \end{enumerate}

% \item[Triples: ]
%     \begin{enumerate}
%         \item Wait for \mathsf{Ok} or \mathsf{Abort} from the adversary. If the adversary sends $\mathsf{Abort}$, send $\mathsf{Abort}$ to all parties and abort. Otherwise choose random values $a^i, b^i \in \mathbb{Z}_p$ for $i \notin A$.
%         \item For each corrupt party $P_i, i \in A$, the environment specifies shares $a^i, b^i$
%         \item Set $a = \sum^i a^i, b = \sum^i b^i$ and $c = a \cdot b$ 
%         \item For each corrupt party $P_i, i \in A$, the environment specifies shares $c^i$.
%         \item For each honest party $P_i, i\notin A$ randomly choose $c^i$ subject to $c = \sum^i c^i$ 
%         \item Run Macros $\mathsf{GenMAC(a_1, \hdots , a_n, \alpha), GenMAC(b_1, \hdots , b_n, \alpha)}$ and $\mathsf{GenMAC(c_1, \hdots , c_n, \alpha)}$\\
%     \end{enumerate}

% \item[Squares: ]
%     \begin{enumerate}
%         \item Hmm
%     \end{enumerate}

% \item[Bits: ]
%     \begin{enumerate}
%         \item Hmm
%     \end{enumerate}
\end{description}
\end{Boxfig}



==> Sections/preliminaries.tex <==

\section{Preliminaries}\label{sec:preliminaries}

We first begin by formalizing the adversarial model. We provide malicious security with abort. In other words, we consider a static malicious adversary who corrupts at most 1 of the participating servers. We aim to guarantee computation privacy as well as correctness of execution. 

Private training of neural networks without batch normalization is extremely difficult and requires significant pre-training. To truly enable private deep learning, efficient protocols for batch normalization are required. 
